AI for Climate Finance: Agentic Retrieval and Multi-Step Reasoning for Early Warning System Investments

Tracking financial investments in climate adaptation is a complex and expertise-intensive task, particularly for Early Warning Systems (EWS), which lack standardized financial reporting across multilateral development banks (MDBs) and funds. To address this challenge, we introduce an LLM-based agentic AI system that integrates contextual retrieval, fine-tuning, and multi-step reasoning to extract relevant financial data, classify investments, and ensure compliance with funding guidelines. Our study focuses on a real-world application: tracking EWS investments in the Climate Risk and Early Warning Systems (CREWS) Fund. We analyze 25 MDB project documents and evaluate multiple AI-driven classification methods, including zero-shot and few-shot learning, fine-tuned transformer-based classifiers, chain-of-thought (CoT) prompting, and an agent-based retrieval-augmented generation (RAG) approach. Our results show that the agent-based RAG approach significantly outperforms other methods, achieving 87\% accuracy, 89\% precision, and 83\% recall. Additionally, we contribute a benchmark dataset and expert-annotated corpus, providing a valuable resource for future research in AI-driven financial tracking and climate finance transparency.

==> latex_table.tex <==
\begin{longtable}{lllllllll}
\toprule
                                          Fund &                                  Project ID &                                          Component &               Outcome/Expected Outcome, Objectives &                              Output /sub-component &                        Activity / Output indicator &    Page number &       Amount &        Label \\
\midrule
\endfirsthead

\toprule
                                          Fund &                                  Project ID &                                          Component &               Outcome/Expected Outcome, Objectives &                              Output /sub-component &                        Activity / Output indicator &    Page number &       Amount &        Label \\
\midrule
\endhead
\midrule
\multicolumn{9}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
Climate Risk and Early Warning Systems (CREWS) &                        CREWS-ASW-\_-Maldives &                                                NaN & enhancing understanding of the status of risk k... &                                                NaN & enhancing understanding of the status of risk k... &            NaN &        20000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS-ASW-\_-Maldives &                                                NaN & enhancing understanding of the status of risk k... &                                                NaN & : Support on institutionalization of disaster d... &            NaN &        60000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS-ASW-\_-Maldives &                                                NaN & enhancing understanding of the status of risk k... &                                                NaN & reinforcement of feedback mechanisms from subna... &            NaN &        50000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS-ASW-\_-Maldives &                                                NaN & enhancing understanding of the status of risk k... &                                                NaN & : Coordination and operation of the new Risk Wo... &            NaN &        20000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS-ASW-\_-Maldives &                                                NaN & enhancing understanding of the status of risk k... &                                                NaN & Knowledge product development and training (in ... &            NaN &        65000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS-ASW-\_-Sierra Leone & Information ecosystem mapping to improve the de... &                                                NaN &                                                NaN & Baseline assessment and Information Ecosystems ... &           2, 5 &        70000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS-ASW-\_-Sierra Leone & Information ecosystem mapping to improve the de... &                                                NaN &                                                NaN & Final user needs assessment after the rainy sea... &           2, 5 &        35000 &      Pillar3 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS-ASW-\_-Sierra Leone &         Capacity building and technical assistance &                                                NaN &                                                NaN & Capacity building/training through partnering w... &           2, 5 &        60000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS-ASW-\_-Sierra Leone &         Capacity building and technical assistance &                                                NaN &                                                NaN & Technical assistance to improve/develop critica... &           2, 6 &        60000 &      Pillar4 \\
Climate Risk and Early Warning Systems (CREWS) &                          CREWS-ASW-03-Tonga & Systems assessment, analysis and design of appl... &                                                NaN & Report on assessment and analysis of existing, ... &                                                NaN &           4, 5 &        21000 &      Pillar3 \\
Climate Risk and Early Warning Systems (CREWS) &                          CREWS-ASW-03-Tonga & Initial development and setup of applications -... &                                                NaN & Initial version of applications and database de... &                                                NaN &           4, 5 &        21000 &      Pillar3 \\
Climate Risk and Early Warning Systems (CREWS) &                          CREWS-ASW-03-Tonga & Training through workshops and consultations fo... &                                                NaN & People in all 121 communities are trained to us... &                                                NaN &           4, 5 &        21000 &      Pillar3 \\
Climate Risk and Early Warning Systems (CREWS) &                          CREWS-ASW-03-Tonga & Training through workshops and consultations fo... &                                                NaN & TMS and NEMO personal are trained to use, trial... &                                                NaN &           4, 5 &        21000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                          CREWS-ASW-03-Tonga & Training through workshops and consultations fo... &                                                NaN & Authorized TMS and district and villages? offic... &                                                NaN &           4, 5 &        21000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                          CREWS-ASW-03-Tonga & Training through workshops and consultations fo... &                                                NaN & TMS, NEMO and other government and first respon... &                                                NaN &           4, 5 &        42000 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                          CREWS-ASW-03-Tonga &                                                NaN &                                                NaN & Applications final testing, updating and enhanc... &                                                NaN &              5 &        42000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS-ASW-05-Vanuatu & To organize Implementing Arrangement (IA) betwe... & Assess communities? capacity to prepare and res... & Action?s implementation arrangement established... &                                                NaN &        2, 4, 5 &        43000 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS-ASW-05-Vanuatu & To organize national consultation workshop to p... & Assess communities? capacity to prepare and res... & Organize national consultation workshop. Data a... &                                                NaN &        2, 4, 5 &        60000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS-ASW-05-Vanuatu & To present draft report to communities and stak... & Assess communities? capacity to prepare and res... & Draft report presented to communities and other... &                                                NaN &        2, 4, 5 &        48000 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS-ASW-05-Vanuatu & To prepare final report, scientific paper/journ... & Assess communities? capacity to prepare and res... & Final report, scientific paper/journal and awar... &                                                NaN &        2, 4, 5 &        49000 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                           CREWS-ASW-06-Cuba & Assessment of national capacities and requireme... &                                                NaN &                                                NaN & Assessment on climate, hydrometeorology and war... &            NaN &      30,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                           CREWS-ASW-06-Cuba & Assessment of national capacities and requireme... &                                                NaN &                                                NaN & Brief project proposal, including action plan w... &            NaN &      10,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                           CREWS-ASW-06-Cuba & Assessment of national capacities and requireme... &                                                NaN &                                                NaN &          Validation workshop and user consultation &            NaN &        10000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                           CREWS-ASW-06-Cuba & Improve the production of meteorological, clima... &                                                NaN &                                                NaN & Improving the process to generate weather forec... &            NaN &        90000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                           CREWS-ASW-06-Cuba & Improve the production of meteorological, clima... &                                                NaN &                                                NaN & Design a plan to develop and implement a platfo... &            NaN &        30000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                           CREWS-ASW-06-Cuba & Improve the production of meteorological, clima... &                                                NaN &                                                NaN & Improve hydrological forecasting products for w... &            NaN &        50000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS/ASW/08/Guinea  & Support the implementation of technical equipme... & Agence National Meteorologie of Guinea has the ... &                                                NaN &                            Renting of the property &            NaN &       167000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS/ASW/08/Guinea  & Support the implementation of technical equipme... & Agence National Meteorologie of Guinea has the ... &                                                NaN &                               Internet connections &            NaN &         6000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS/ASW/08/Guinea  & Advisory services in order to solidify the inst... & Agence National Meteorologie of Guinea has suff... & Institutional strengthening activities for the ... & Support for a strategic plan and legal document... &            NaN &        24239 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS/ASW/08/Guinea  & Advisory services in order to solidify the inst... & Agence National Meteorologie of Guinea has suff... &                                                NaN & Develop a financial/business plan for the susta... &            NaN &        12000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS/ASW/08/Guinea  & Advisory services in order to solidify the inst... & Agence National Meteorologie of Guinea has suff... &                                                NaN &   Elaborate staff statutes, operational procedures &            NaN &        12000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                          CREWS-Cproj-01-DRC & Institutional and regulatory strengthening, cap... & will invest in strengthening institutional setu... &                                                NaN & (i) Reinforce the legal and regulatory framewor... &            NaN &      2305000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                          CREWS-Cproj-01-DRC & Modernization of equipment, facilities and infr... & will finance: i) hydrological and meteorologica... &                                                NaN & (i) Hydrological and meteorological monitoring ... &            NaN &      4568000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                          CREWS-Cproj-01-DRC & Improvement of hydromet information service del... & will provide technical assistance for delivery ... &                                                NaN & (i) Establishing a national framework for clima... &            NaN &      1842500 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                          CREWS-Cproj-01-DRC & Improvement of hydromet information service del... & will provide technical assistance for delivery ... &                                                NaN & (ii) Develop and deliver customized products an... &            NaN &      1842500 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS-Cproj-02-Mali & Institutional Strengthening, Capacity Building ... & strengthening institutional setup and building ... & : i) reinforcing the legal and regulatory frame... &                                                NaN &              4 &     11411000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS-Cproj-02-Mali & Modernization of observation infrastructure and... &                                                NaN & i) hydrological and meteorological monitoring n... &                                                NaN &              4 &     11411000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS-Cproj-02-Mali &       Enhancement of Service Delivery to End-Users & technical assistance for delivery of more accur... & (i) defining of requirements and developing fee... &                                                NaN &              4 &  11,411,000  &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                      CREWS/Cproj/03/Burkina &                                      Basic systems & Reinforcement of DGM and DGER technical capabil... & Assessment of observation network processes and... &                                                NaN &           4, 5 &     189,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                      CREWS/Cproj/03/Burkina &                                      Basic systems & Reinforcement of DGM and DGER technical capabil... & Data base improvement. Consolidation of CLIDATA... &                                                NaN &           4, 6 &     189,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                      CREWS/Cproj/03/Burkina &                                      Basic systems & Reinforcement of DGM and DGER technical capabil... & Short term forecast capabilities. Enhancing ava... &                                                NaN &           4, 7 &       189000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                      CREWS/Cproj/03/Burkina &                                      Basic systems & Reinforcement of DGM and DGER technical capabil... & Sub-Seasonal to seasonal forecast. Development ... &                                                NaN &           4, 8 &       189000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                      CREWS/Cproj/03/Burkina &                                      Basic systems & Reinforcement of DGM and DGER technical capabil... & Analysis and nowcasting tools. Early Warning ca... &                                                NaN &           4, 9 &     189,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                      CREWS/Cproj/03/Burkina &        Support to Early Warning System development & Weather and climate information will be transla... & Risk information and forecast products for floo... &                                                NaN &           6, 7 &     322,500  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                      CREWS/Cproj/03/Burkina &        Support to Early Warning System development & Weather and climate information will be transla... & Risk information and forecast products for agri... &                                                NaN &              7 &     322,500  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                      CREWS/Cproj/03/Burkina &                        Institutional strengthening &                 Long term development plan for DGM & Short-term, project-level, investments are sign... &                                                NaN &              7 &      50,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                      CREWS/Cproj/03/Burkina &                                 Project Management &                                     Implementation & The project will finance the following activiti... &                                                NaN &              7 &       200000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                      CREWS/Cproj/03/Burkina &                          Monitoring and Evaluation & independent impact assessment of the informatio... &                                                NaN &                                                NaN &              8 &     100,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/Cproj/10/Afghanistan & Enhancement of the service delivery system to d... & The consultations with stakeholders have clearl... & Developing and implementing a National Strategy... & Development of a Strategy for Service Delivery ... &          7, 10 &     228,571  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/Cproj/10/Afghanistan & Enhancement of the service delivery system to d... & The consultations with stakeholders have clearl... & Establishing a collaborative approach between A... & Establishment of a national joint flood forecas... &       7, 8, 10 &     228,571  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/Cproj/10/Afghanistan & Enhancement of the service delivery system to d... & The consultations with stakeholders have clearl... & Enhancing public weather, climate and hydrologi... & Provide technical support for DRM/EW in the ope... &          8, 10 &     228,571  &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/Cproj/10/Afghanistan & Enhancement of the service delivery system to d... & The consultations with stakeholders have clearl... & Enhancing public weather, climate and hydrologi... & Strengthening of Early Warning dissemination an... &       8, 9, 10 &     228,571  &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/Cproj/10/Afghanistan & Enhancement of the service delivery system to d... & The consultations with stakeholders have clearl... & Enhancing agro-met services including, developi... & Provide technical support for the implementatio... &       8, 9, 10 &     228,571  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/Cproj/10/Afghanistan & Enhancement of the service delivery system to d... & The consultations with stakeholders have clearl... & Enhancing agro-met services including, developi... & Development of a drought monitoring programme (... &       8, 9, 11 &     228,571  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/Cproj/10/Afghanistan & Enhancement of the service delivery system to d... & The consultations with stakeholders have clearl... & Introducing a Quality Management System (QMS) f... & Introduction of a QMS for AMD (including aerona... &       8, 9, 12 &     228,571  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/Cproj/10/Afghanistan &  Institutional Strengthening and capacity building & This component will aim to improve the performa... & Reinforce the legal and institutional framework... & Strengthening of the institutional and legal fr... &         10, 11 &     250,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/Cproj/10/Afghanistan &  Institutional Strengthening and capacity building & This component will aim to improve the performa... & The development of a Concept of Operations (CON... &                            Development of a CONOPS &         10, 11 &     250,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/Cproj/10/Afghanistan &  Institutional Strengthening and capacity building & This component will aim to improve the performa... & Building capacity to improve the sustainability... & Delivery of the technical capacity and competen... &         10, 11 &     250,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/Cproj/10/Afghanistan &  Institutional Strengthening and capacity building & This component will aim to improve the performa... & Building project management capacity (of AMD) I... & Development of project management, procurement ... &             11 &     250,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/Cproj/10/Afghanistan & Strengthening data management and forecasting c... &                                                NaN & Building a readily accessible digital hydrologi... & Development of a platform that is unifying, col... &         11, 12 &     273,333  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/Cproj/10/Afghanistan & Strengthening data management and forecasting c... &                                                NaN & Developing a modern impact-based weather foreca... & Strengthening the technical capacity and establ... &         12, 13 &     273,333  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/Cproj/10/Afghanistan & Strengthening data management and forecasting c... &                                                NaN & Enhancing Flash Flood forecasting and alerting ... &            Development of impact-based forecasting &             13 &     273,333  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS-Cproj-11-Chad & Strengthening Hydrological and Meteorological S... &                                                NaN & Provision of scientific and technical advice to... &                                                NaN &              4 &     300,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS-Cproj-11-Chad & Strengthening Hydrological and Meteorological S... &                                                NaN & Support to climate watch service for (i) enhanc... &                                                NaN &              4 &     200,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS-Cproj-11-Chad & Strengthening Hydrological and Meteorological S... &                                                NaN & Support the design and carrying out of piloting... &                                                NaN &              4 &     200,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS-Cproj-11-Chad & Strengthening Hydrological and Meteorological S... &                                                NaN & Support to the development of a capacity buildi... &                                                NaN &              5 &     300,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS-Cproj-11-Chad & Strengthening Hydrological and Meteorological S... &                                                NaN & Direct support (transfer of funds to beneficiar... &                                                NaN &              5 &     327,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS-Cproj-11-Chad & Strengthening Hydrological and Meteorological S... &                                                NaN & Undertake a capacity assessment, strategic deve... &                                                NaN &              5 &     100,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS-Cproj-11-Chad & Strengthening of end user?s capacity for servic... &                                                NaN & Design and carry out Technical assistance for C... &                                                NaN &              5 &     300,000  &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS-Cproj-11-Chad & Strengthening of end user?s capacity for servic... &                                                NaN & Support the design and carrying out of piloting... &                                                NaN &              5 &     800,000  &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS-Cproj-11-Chad & Strengthening of end user?s capacity for servic... &                                                NaN & Institutional support and training in contingen... &                                                NaN &              5 &     300,000  &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS/CProj/12/Togo & Strengthening hydrological and meteorological s... &                                                NaN & Provision of scientific and technical advice to... &                                                NaN &              4 &     200,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS/CProj/12/Togo & Strengthening hydrological and meteorological s... &                                                NaN & Support to climate watch service for enhanced s... &                                                NaN &              4 &     200,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS/CProj/12/Togo & Strengthening hydrological and meteorological s... &                                                NaN & Support to the development of a capacity buildi... &                                                NaN &           4, 5 &     200,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS/CProj/12/Togo & Strengthening hydrological and meteorological s... &                                                NaN & Support the design and carrying out of piloting... &                                                NaN &              5 &     173,000  &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS/CProj/12/Togo & Strengthening hydrological and meteorological s... &                                                NaN & Direct support (transfer of funds to beneficiar... &                                                NaN &              5 &     200,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS/CProj/12/Togo & Strengthening hydrological and meteorological s... &                                                NaN & Undertake a capacity assessment, strategic deve... &                                                NaN &              5 &     100,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS/CProj/12/Togo & Civil protection, emergency management, disaste... &                                                NaN & Support the design and carrying out of piloting... & Development of hydrologic modelling for risk as... &              5 &     250,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS/CProj/12/Togo & Civil protection, emergency management, disaste... &                                                NaN & Support the design and carrying out of piloting... & Vulnerability and exposure mapping to flood ris... &              5 &     150,000  &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS/CProj/12/Togo & Civil protection, emergency management, disaste... &                                                NaN & Support the design and carrying out of piloting... & Support to the development of multi-hazard risk... &              5 &     150,000  &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS/CProj/12/Togo & Civil protection, emergency management, disaste... &                                                NaN & Support the design and carrying out of piloting... & Support to community engagement and woman group... &              5 &     200,000  &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS/CProj/12/Togo & Civil protection, emergency management, disaste... &                                                NaN & Support for development of national operational... &                                                NaN &           5, 6 &     100,000  &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                         CREWS/CProj/12/Togo & Civil protection, emergency management, disaste... &                                                NaN & Institutional support and training in contingen... &                                                NaN &              6 &     200,000  &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS/CProj/13/Hati & Enhanced UHM to deliver high quality services t... &                                                NaN & Quality Management System developed and maintained & Host high level finalization and validation wor... &             14 &     284,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS/CProj/13/Hati & Enhanced UHM to deliver high quality services t... &                                                NaN & Technical capacities of UHM to provide forecast... & Conduct technical workshops; Improve calibratio... &             14 &     284,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS/CProj/13/Hati &     Improved Hydro-meteorological Warning \textbackslash nSystem &                                                NaN &  National Coordination Mechanism \textbackslash nstrengthened... & Conduct consultations to identify priority user... &             14 &      50,000  & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS/CProj/13/Hati &     Improved Hydro-meteorological Warning \textbackslash nSystem &                                                NaN & Early Warning Services developed and accessible... & Conduct consultations with agriculture sector t... &             14 &      50,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                        CREWS/CProj/13/Hati & Enhanced preparedness and response \textbackslash ncapacities... &                                                NaN & Preparedness and Response plans strengthened \textbackslash n... & Identify and conduct risk assessment of pilot c... &             14 &     119,034  &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening the production of climate service... &                                                NaN &    Strengthening the provision of climate services & Enhancing National Climate Services (ENACTS) se... &       6, 7, 13 &     150,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening the production of climate service... &                                                NaN &    Strengthening the provision of climate services & Roll-out National Climate Outlook Forums in Malawi &       6, 7, 13 &      50,000  & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening the production of climate service... &                                                NaN &    Strengthening the provision of climate services & Strengthening of the production of climate serv... &       6, 7, 13 &     200,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening the production of climate service... &                                                NaN &    Strengthening the provision of climate services & Development of M\&E framework for monitoring the... &       6, 7, 13 &      70,000  & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening the production of climate service... &                                                NaN & Strengthening regional coordination and coopera... & Adapt and Calibrate the Composite Drought Index... &       6, 7, 13 &     195,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening the production of climate service... &                                                NaN & Strengthening regional coordination and coopera... & Support DCCMS with a semiautomatic, easy to run... &       6, 7, 13 &     150,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening the production of climate service... &                                                NaN & Strengthening regional coordination and coopera... & Design of a soilÿmoistureÿmonitoring network fo... &       6, 7, 13 &      90,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening the production of climate service... &                                                NaN & Strengthening regional coordination and coopera... & Measure effectiveness of EWS against indicators... &       6, 7, 13 &      80,000  & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening the production of climate service... &                                                NaN & Enhancement of Flood early warning system in th... & Enhancement of the Operational Decision Support... &       6, 7, 14 &     180,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening the production of climate service... &                                                NaN & Enhancement of Flood early warning system in th... & Training and capacity building of the technical... &       6, 7, 14 &      80,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening the production of climate service... &                                                NaN & Enhancement of Flood early warning system in th... & Training and awareness of all users: National, ... &       6, 7, 14 &      80,000  &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening early warning dissemination, prep... &                                                NaN & Strengthening early warning dissemination and p... & Support the development of a gender sensitive a... &       6, 7, 14 &     262,035  &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening early warning dissemination, prep... &                                                NaN & Strengthening urban flood risk management in th... & Probabilistic Flood risk assessments for the ci... &       6, 8, 14 &     250,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening early warning dissemination, prep... &                                                NaN & Strengthening urban flood risk management in th... & Formulation of flood risk management strategies... &       6, 8, 14 &     150,000  &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening early warning dissemination, prep... &                                                NaN & Strengthening urban flood risk management in th... & Support the consolidation of the urban disaster... &       6, 9, 14 &      80,000  &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening early warning dissemination, prep... &                                                NaN &  Operationalization of the Risk Financing Strategy & Support the design and establishment of the Dis... &       6, 9, 14 &     100,000  &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening early warning dissemination, prep... &                                                NaN &  Operationalization of the Risk Financing Strategy & Technical inputs to support decision making on ... &       6, 9, 14 &      90,000  &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi & Strengthening early warning dissemination, prep... &                                                NaN &  Operationalization of the Risk Financing Strategy & Exchange, awareness, and training of Risk Finan... &       6, 9, 14 &      50,000  &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi &                                  Capacity Building &                                                NaN &                               Capacity Development & Training for NMHS staff and users on basic syst... &       6, 9, 14 &     205,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                       CREWS/CProj/14/Malawi &                                  Capacity Building &                                                NaN &                               Capacity Development & Simulation exercise for DoDMA and DCCMS staff a... &       6, 9, 14 &     100,000  &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Anm's and CERD's service delivery improved, inc... &                                                NaN & Institutional and human capacity of ANM and CER... & Review ANM's current National Strategic Plan fo... &         16, 24 &      16,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Anm's and CERD's service delivery improved, inc... &                                                NaN & Institutional and human capacity of ANM and CER... & Develop National Strategic Plan and Framework f... &         16, 24 &      25,000  & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Anm's and CERD's service delivery improved, inc... &                                                NaN & Institutional and human capacity of ANM and CER... & Development of a national communication protoco... &         16, 24 &      30,000  &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Anm's and CERD's service delivery improved, inc... &                                                NaN & Institutional and human capacity of ANM and CER... & Education and training of staff from ANM and CE... &         16, 24 &     100,000  & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Anm's and CERD's service delivery improved, inc... &                                                NaN & Enhanced capacity by ANM to provide weather and... & Improving the observational and forecasting cap... &         16, 24 &      60,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Anm's and CERD's service delivery improved, inc... &                                                NaN & Strengthened co-production between producers an... & Establish the first National Climate Outlook Fo... &         16, 24 &      30,000  & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Anm's and CERD's service delivery improved, inc... &                                                NaN &                                                NaN & Socio-economic benefits analysis of hydrometeor... &         16, 24 &      30,000  & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Anm's and CERD's service delivery improved, inc... &                                                NaN &                                                NaN & Develop hydrological status and outlook system ... &         16, 25 &     300,000  &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Risk Information to guide early warning systems... &                                                NaN & Improved access to risk information through enh... & Conduct EW4All Pillar 1 workshop on the use of ... &     16, 25, 26 &     175,000  &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Risk Information to guide early warning systems... &                                                NaN &                                                NaN & Build and enhance national, sub-national, and l... &     16, 25, 26 &       190000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Risk Information to guide early warning systems... &                                                NaN & Strengthened National capacities in Djibouti fo... & Build national capacity for developing, using a... &     16, 26, 27 &       150000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Risk Information to guide early warning systems... &                                                NaN &                                                NaN & Support the coordination of the National DRR pl... & 16, 27, 28, 29 &       227333 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Risk Information to guide early warning systems... &                                                NaN &                                                NaN & Strengthen National Climate Outlook Forums (NCO... & 16, 27, 28, 29 &       113667 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Information and communication technologz streng... &                                                NaN & Development of ANM's and CERD's technical and c... &                            Website upgrade for ANM &             29 &        30000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Information and communication technologz streng... &                                                NaN & Development of ANM's and CERD's technical and c... &        Purchase of ICT equipment for ANM and CERDÿ &             29 &        60000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Information and communication technologz streng... &                                                NaN & Enhancing monitoring and observational data exc... & Support Data Rescue at ANM and CERD, and renewa... &             29 &        75000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Information and communication technologz streng... &                                                NaN & Enhancing monitoring and observational data exc... & Strengthen data management (both CERD and ANM) ... &             29 &       130000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Information and communication technologz streng... &                                                NaN & Enhancing monitoring and observational data exc... &         Technical support for WIGOS implementation &             29 &        70000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Information and communication technologz streng... &                                                NaN &                      Communication of EWS Improved & Common Alert Protocol (CAP) implementation and ... &             29 &        30000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Information and communication technologz streng... &                                                NaN & Enhancement of basic observing and forecasting ... & Procurement and deployment of automatic weather... &             29 &       200000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Information and communication technologz streng... &                                                NaN & Enhancement of basic observing and forecasting ... & Procurement, rehabilitation and deployment of P... &           29.0 &        30000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Information and communication technologz streng... &                                                NaN & Enhancement of basic observing and forecasting ... & Development of guidance and plan on sustainabil... &           30.0 &        10000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Preparedness and response plans with operationa... &                                                NaN & Ensure warning communication and dissemination ... & CBEWS implemented and preparedness and response... &           30.0 &       170000 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Preparedness and response plans with operationa... &                                                NaN &                                                NaN & Early warning dissemination reinforced through ... &           30.0 &        20000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Knowledge products and awareness programmes on ... &                                                NaN &      Knowledge products and publications developed & develop and design communication and knowledge ... &           30.0 &      15,000  & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Gender-sensitive training, capacity building pr... &                                                NaN &                mainstreaming gender and disability & Development and provision of national trainings... &           30.0 &        20000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/CProj/16/Djiboutiÿ & Gender-sensitive training, capacity building pr... &                                                NaN &                mainstreaming gender and disability & National roll out of the Inclusive early warnin... &           30.0 &        30000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                        Data, products and exchange &                                                NaN & Assessment of observation network processes and... & Contacting observation network owners (mostly  ... &            NaN &        20000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                        Data, products and exchange &                                                NaN &                                                NaN & Preparation of a plan to make observations avai... &            NaN &        20000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                        Data, products and exchange &                                                NaN &                              Data base improvement & Setting-up the WACA\&D system for West-Africa (s... &            NaN &       200000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                        Data, products and exchange &                                                NaN &                                                NaN & Hardware: Purchase \& shipment of computer to ru... &            NaN &        15000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                        Data, products and exchange &                                                NaN &                                                NaN & Climsoft update for implementation at observati... &            NaN &         8000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                        Data, products and exchange &                                                NaN & Set-up of a data base on impacts of extreme eve... & identify priorities and needs of stakeholders f... &            NaN &         8000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                        Data, products and exchange &                                                NaN &                                                NaN & Identify existing initatives for collecting and... &            NaN &         8000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                        Data, products and exchange &                                                NaN &                                                NaN & Identify, and develop standards for information... &            NaN &         8000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                        Data, products and exchange &                                                NaN &                                                NaN & Develop and implement process for operational i... &            NaN &        16000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                        Data, products and exchange &                                                NaN &                                                NaN & evaluate and optimize user interface for analys... &            NaN &         8000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                        Data, products and exchange &                                                NaN & Early Warning system integration and seamless s... &                One user form in each CREWS country &            NaN &        37500 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                        Data, products and exchange &                                                NaN &                                                NaN & One training in each CREWS country to build cap... &            NaN &        37500 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                   Analysis and climate watch tools &                                                NaN &                                                NaN &                 identify priorities of stakeholder &            NaN &         8000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                   Analysis and climate watch tools &                                                NaN &                                                NaN & development of CM SAF satellite- and GPCC-based... &            NaN &        16000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                   Analysis and climate watch tools &                                                NaN &                                                NaN & identifing optimal procedure(s) for generating ... &            NaN &        16000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                   Analysis and climate watch tools &                                                NaN &                                                NaN & developing processes for generating the CM prod... &            NaN &        32000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                   Analysis and climate watch tools &                                                NaN &                                                NaN & evaluating and improving performance and qualit... &            NaN &         8000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                   Analysis and climate watch tools &                                                NaN &                                                NaN &                    operationalizing the procedures &            NaN &        24000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                   Analysis and climate watch tools &                                                NaN &                                                NaN &            CWS workshop with regional stakeholders &            NaN &         8000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                   Analysis and climate watch tools &                                                NaN &                                                NaN & designing and setting up a CWS decision making ... &            NaN &        24000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa & Improved short- to medium-range forecast capabi... &                                                NaN &                                                NaN & CREWS / SWFDP Training Workshops on Severe Weat... &            NaN &       130000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa & Improved short- to medium-range forecast capabi... &                                                NaN &                                                NaN & RSMC Dakar Training Desk (for 2 forecasters/PWS... &            NaN &        10000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa & Improved short- to medium-range forecast capabi... &                                                NaN &                                                NaN & In-country visits (2 countries per year) to gat... &            NaN &        20000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa & Improved short- to medium-range forecast capabi... &                                                NaN &                                                NaN & Based on mission assessment reports, develop na... &            NaN &        20000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa & Improved short- to medium-range forecast capabi... &                                                NaN &                                                NaN & Support participants from SWFDP countries at th... &            NaN &        14500 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                                     Flood forecast &                                                NaN &                                                NaN &                          Initial Planning Meeting  &            NaN &       35,000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                                     Flood forecast &                                                NaN &                                                NaN &          Development of Geomorphological relations &            NaN &       20,000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                                     Flood forecast &                                                NaN &                                                NaN &                 Verification of Basin delineations &            NaN &       10,000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                                     Flood forecast &                                                NaN &                                                NaN & Initial development and implementation of  West... &            NaN &      250,000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                                     Flood forecast &                                                NaN &                                                NaN &                       Steering Committee Meeting 1 &            NaN &       25,000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                                     Flood forecast &                                                NaN &                                                NaN &                     On line FFGS training (Step 2) &            NaN &       10,000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                                     Flood forecast &                                                NaN &                                                NaN &               Operational Training at HRC (Step 3) &            NaN &       60,000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                                     Flood forecast &                                                NaN &                                                NaN &              Regional Operations Training (Step 4) &            NaN &       25,000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                                     Flood forecast &                                                NaN &                                                NaN &                   Sustainability training (Step 5) &            NaN &       25,000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                                     Flood forecast &                                                NaN &                                                NaN & Purchase of FFGS servers and shipment to DR Nig... &            NaN &       35,000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                                     Flood forecast &                                                NaN &                                                NaN &                         Maintain the system at HRC &            NaN &       30,000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                                     Flood forecast &                                                NaN &                                                NaN & Onsite installation of FFGS servers and It trai... &            NaN &       15,000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                                     Flood forecast &                                                NaN &                                                NaN &                                Operations Supports &            NaN &       35,000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                   Subseasonal to seasonal forecast &                                                NaN &                                                NaN & Sub-seasonal-to-seasonal prediction, developing... &            NaN &       100000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/02/Western Africa &                   Subseasonal to seasonal forecast &                                                NaN &                                                NaN & Pilot services on early warnings for agricultur... &            NaN &        50000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa &                        Data, products and exchange &                                                NaN &                                                NaN & Analysis of observation networks and data archi... &            NaN &        15000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa &                        Data, products and exchange &                                                NaN &                                                NaN & Setting-up the West Africa Climate Assessment a... &            NaN &        15000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa &                        Data, products and exchange &                                                NaN &                                                NaN & Setting-up an extreme event catalogue (e.g KRONER) &            NaN &        10000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa &                        Data, products and exchange &                                                NaN &                                                NaN & Harmonized approaches to early warning and rapi... &            NaN &        10000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa &                   Analysis and climate watch tools &                                                NaN &                                                NaN &        Enhancing Climate Watch Advisories (CWAs) - &            NaN &        10000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa & Improved short- to medium-range forecast capabi... &                                                NaN &                                                NaN & Improved short term and severe weather forecast... &            NaN &       900000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa &                                     Flood forecast &                                                NaN &                                                NaN & Flood forecasting extended to all ECOWAS and PR... &            NaN &       900000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa &                   Subseasonal to seasonal forecast &                                                NaN &                                                NaN & Sub-seasonal to seasonal prediction and regiona... &            NaN &        10000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa &                   Subseasonal to seasonal forecast &                                                NaN &                                                NaN & Sub-seasonal to seasonal forecast tailoring to ... &            NaN &        10000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa &                   Subseasonal to seasonal forecast &                                                NaN &                                                NaN &                 Pilot services on severe drought - &            NaN &        20000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa & Developing a long-term strategy for sustainable... &                                                NaN &                                                NaN & Service delivery strategy and the concept of op... &            NaN &       116667 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa & Developing a long-term strategy for sustainable... &                                                NaN &                                                NaN &                 Public-private engagement strategy &            NaN &       116667 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa & Developing a long-term strategy for sustainable... &                                                NaN &                                                NaN & Piloting the innovative technology in meteorolo... &            NaN &       116667 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa & Improvement of regional training capacity and s... &                                                NaN &                                                NaN & Regional training needs assessment and training... &            NaN &       125000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa & Improvement of regional training capacity and s... &                                                NaN &                                                NaN & Provision of priority key training in West Afri... &            NaN &       125000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa & Community early warning and preparedness planni... &                                                NaN & New/ enhanced weather and early warning informa... &                                                NaN &            NaN &        60000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa & Community early warning and preparedness planni... &                                                NaN &           Enhanced community communication systems &                                                NaN &            NaN &        60000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa & Community early warning and preparedness planni... &                                                NaN & Key infrastructure mapping of vulnerability com... &                                                NaN &            NaN &        60000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa & Community early warning and preparedness planni... &                                                NaN &                        Community capacity building &                                                NaN &            NaN &        60000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa & Community early warning and preparedness planni... &                                                NaN & Development and implementation of training prog... &                                                NaN &            NaN &        60000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa & Detailed design and guidance for establishment ... &                                                NaN & Enhanced weather and climate information produc... &                                                NaN &            NaN &       175000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa & Detailed design and guidance for establishment ... &                                                NaN & Flash Flood guidance system established and ope... &                                                NaN &            NaN &       175000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa & Detailed design and guidance for establishment ... &                                                NaN & Meteorological and hydrological observation str... &                                                NaN &            NaN &       175000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &               CREWS/RProj/03/Western Africa & Detailed design and guidance for establishment ... &                                                NaN &     Improved meteorological data management system &                                                NaN &            NaN &       175000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) & CREWS/RProj/05/Additional Financing Pacific &                                Improved Governance & Strengthened enabling environment for the Regio... & Support the development of bills, legislations,... & Development of template for drafting bills. Dra... &            NaN &       265000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) & CREWS/RProj/05/Additional Financing Pacific &                                Improved Governance &                                                NaN & National Strategic Plans inclusive of costed im... & Review existing or develop new NSPs for meteoro... &            NaN &       285000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) & CREWS/RProj/05/Additional Financing Pacific &                                Improved Governance &                                                NaN & WMO and regional coordination mechanisms for me... & Provide logistical support to the Pacific Meteo... &            NaN &       195000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) & CREWS/RProj/05/Additional Financing Pacific &  Enhanced Product Co-Development and Accessibility &                                                NaN & Integrated and inclusive operational Early Warn... & Develop and implement national integrated and i... &            NaN &       255000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) & CREWS/RProj/05/Additional Financing Pacific &  Enhanced Product Co-Development and Accessibility &                                                NaN & Implementation of a high-resolution NWP mesosca... & Upgrade and enhance FMS and RSMC Nadi's website... &            NaN &       175000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) & CREWS/RProj/05/Additional Financing Pacific &                          Enhanced Service Delivery & Improved quality of accessible services provide... & Support development of Regional ICT Strategy th... & Assess ICT capacity, needs and accessibility re... &            NaN &        90000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) & CREWS/RProj/05/Additional Financing Pacific &                          Enhanced Service Delivery &                                                NaN &           Communication of Early Warning Improved  & Conduct stakeholder consultations, including gr... &            NaN &       103000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) & CREWS/RProj/05/Additional Financing Pacific &                          Enhanced Service Delivery &                                                NaN & National and regional platforms for NMHSs to ex... & Support the hosting of the National Climate Out... &            NaN &       250000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) & CREWS/RProj/05/Additional Financing Pacific &                          Enhanced Service Delivery &                                                NaN & Capacities to detect, monitor and forecast seve... & Capacity building on detecting, monitoring and ... &            NaN &       280000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) & CREWS/RProj/05/Additional Financing Pacific &                          Enhanced Service Delivery &                                                NaN & Community-Based Early Warning System (CB-EWS) i... & Review existing systems in place for accessible... &            NaN &       240000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) & CREWS/RProj/05/Additional Financing Pacific &                          Enhanced Service Delivery &                                                NaN & Communities? response to multi-risk information... & Develop or update existing climate risks maps i... &            NaN &       495000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) & CREWS/RProj/05/Additional Financing Pacific & Enhanced communication and awareness programmes... &                                                NaN &      Knowledge products and publications developed & Develop knowledge products for publication (pee... &            NaN &       109000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) & CREWS/RProj/05/Additional Financing Pacific & Stronger Inclusion  of gender and persons livin... &                                                NaN & Guidance document on mainstreaming gender and d... & Develop guidelines for integrating gender and d... &            NaN &       280000 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Strengthened governance mechanism (policies, st... & National Meteorological and Hydrological Servic... & Drafting of new and / or review \& updating of e... &             28 &        80000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Strengthened governance mechanism (policies, st... &                                                NaN & DRR/Preparedness and response coordination mech... &             28 &        77970 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Strengthened governance mechanism (policies, st... &                                                NaN & Development of National Strategic Plans (for NM... &             28 &       140000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Strengthened governance mechanism (policies, st... &                                                NaN & User Interface Platforms (UIPs) established. Cr... &             28 &       150000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Strengthened governance mechanism (policies, st... &                                                NaN & Support the countries with the development of n... &             29 &       200000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Strengthened governance mechanism (policies, st... &                                                NaN & Improve coordination between the stakeholders t... &             29 &       200000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Strengthened governance mechanism (policies, st... &                                                NaN & Improve coordination and planning for drought m... &         29, 30 &       280000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Increased access and use of global/regional/nat... & Improve discovery, access and use of hydromet d... &             30 &        80000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Increased access and use of global/regional/nat... & Enhance the capacity of the NMHSs to issue fore... &             30 &       322000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Increased access and use of global/regional/nat... & Enhance the access and use of flood and drought... &         30, 31 &       260000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Increased access and use of global/regional/nat... & Incorporate additional functionalities to the S... &             31 &       200000 &     pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Increased access and use of global/regional/nat... & Implement an integrated water resource assessme... &             31 &       100000 &     pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Increased access and use of global/regional/nat... & Improved climate service delivery through opera... &             31 &       250000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Increased access and use of global/regional/nat... & Support the development and/or strengthening of... &             31 &       150000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Increased access and use of global/regional/nat... & Develop new and/ or review and update climate d... &             32 &        50000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Risk information to guide early warning systems... & Review, develop new and/or update existing floo... &             32 &       280000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Risk information to guide early warning systems... & Vulnerability index and profiling capacities fo... &             32 &       100000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Risk information to guide early warning systems... & Enhance capacities for post-disaster impact ass... &          32,33 &       108970 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & NMHS's Information and communication technology... & IT Capacity to support with the activities of t... & Create a Modernization and/or Strategic Plan in... &             33 &       450000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced preparedness and response capability t... & Preparedness and response plans with operationa... & Enhanced understanding of existing hydromet war... &         33, 34 &       240000 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced preparedness and response capability t... & Preparedness and response plans with operationa... & Number of co-developed preparedness and respons... &            NaN &        48970 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced preparedness and response capability t... & Preparedness and response plans with operationa... & Strengthen linkages of early action with shock/... &            NaN &        90000 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced preparedness and response capability t... & Mechanisms considering local and indigenous kno... & In collaboration with NMHSs, DRM authorities at... &         34, 35 &       260000 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced preparedness and response capability t... & Mechanisms considering local and indigenous kno... & Assessment of risk communication, nature hazard... &             35 &        45000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Enhanced preparedness and response capability t... & Mechanisms considering local and indigenous kno... & Support enhancement of warning dissemination an... &         35, 36 &       135000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Improved integration of gender and vulnerable g... & Gender-sensitive and vulnerable people inclusiv... & Government EWS actors and stakeholders? worksho... &             36 &       109000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &              CREWS/RProj/08/South-East Asia &                                                NaN & Improved integration of gender and vulnerable g... & Gender-sensitive and vulnerable people inclusiv... & Guidance document on mainstreaming gender and d... &             36 &        98970 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Institutional and human capacities in regional ... &                                                NaN & Improving regional services to support countrie... & Improving the quality and availability of obser... &         22, 23 &       250000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Institutional and human capacities in regional ... &                                                NaN & Improving regional services to support countrie... & Joint regional training on access and use of da... &             23 &       135000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Institutional and human capacities in regional ... &                                                NaN & Improving regional services to support countrie... & Scale up of good practices and processes (from ... &             23 &       214000 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Institutional and human capacities in regional ... &                                                NaN & Improving regional services to support countrie... & Comprehensive understanding of user needs that ... &             23 &       128000 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Institutional and human capacities in regional ... &                                                NaN & Improving regional services to support countrie... & Enhancing regional capacity to produce and deli... &             24 &       395000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Institutional and human capacities in regional ... &                                                NaN & Improving regional services to support countrie... & Develop hydrological status assessments and out... &         24, 25 &       150000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Institutional and human capacities in regional ... &                                                NaN & Improving regional services to support countrie... & Socio-economic cost benefit study a. Finally, a... &             25 &       300000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Institutional and human capacities in regional ... &                                                NaN & Strengthening regional coordination and coopera... & SOPs aligned to the MHEWS framework piloted in ... &             25 &       100000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Institutional and human capacities in regional ... &                                                NaN & Strengthening regional coordination and coopera... & Establish regional platform for coordination of... &         25, 26 &       242000 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Institutional and human capacities in regional ... &                                                NaN & Strengthening regional coordination and coopera... & Increase collaboration across NMHS?s through re... &             26 &       100000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Institutional and human capacities in regional ... &                                                NaN & Strengthening regional coordination and coopera... & Development of strategic priorities and / or re... &             26 &       110000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Strengthen impact-based Early Warning Services ... &                                                NaN & Strengthening National Risk Data Ecosystems in ... & Strengthening National Risk Data Ecosystems in ... &             26 &       480000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Strengthen impact-based Early Warning Services ... &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Upgrade the Weather and Climate Data Management... &         26, 27 &       285000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Strengthen impact-based Early Warning Services ... &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & ECMWF EcChart licenses renewed, and relevant tr... &             27 &        24000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Strengthen impact-based Early Warning Services ... &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Upgrade NMHSs Public Weather Services infrastru... &             27 &        76000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Strengthen impact-based Early Warning Services ... &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Increased capacity to access and use data excha... &             27 &       330000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Strengthen impact-based Early Warning Services ... &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Assessing the Uganda National Meteorological Au... &             27 &        50000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Strengthen impact-based Early Warning Services ... &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Improving the capacity of UNMA to generate, cus... &             27 &       300000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Strengthen impact-based Early Warning Services ... &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Upgrade of tele-conferencing facilities (Uganda... &             27 &        90000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Strengthen impact-based Early Warning Services ... &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & Development of targeted impact-based early warn... &             28 &       100000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Strengthen impact-based Early Warning Services ... &                                                NaN & Enhanced capacity of NMHSs to provide forecasts... & IBEWS service for Uganda, Kenya, South Sudan an... &             28 &       500000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Strengthen impact-based Early Warning Services ... &                                                NaN & Knowledge products and awareness programmes dev... & Public awareness of weather and use of daily ma... &             28 &        85000 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & Strengthen impact-based Early Warning Services ... &                                                NaN & Knowledge products and awareness programmes dev... & Development of improved community disaster cont... &             28 &       100000 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa &     STRENGTHENING NATIONAL CAPABILITIES IN BURUNDI &                                                NaN &                          Institutional development & Assessment of hydromet monitoring network, earl... &             29 &       150000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa &     STRENGTHENING NATIONAL CAPABILITIES IN BURUNDI &                                                NaN &                          Institutional development & Improving the capacity of IGEBU to generate, cu... &         29, 30 &       250000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa &     STRENGTHENING NATIONAL CAPABILITIES IN BURUNDI &                                                NaN &                          Institutional development & Upgrade of tele-conferencing facilities (Burund... &             30 &        20000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa &     STRENGTHENING NATIONAL CAPABILITIES IN BURUNDI &                                                NaN &                          Institutional development & Strengthening National Risk Data Ecosystems in ... &             30 &        10000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & STRENGTHENING NATIONAL CAPABILITIES IN SOUTH SUDAN &                                                NaN &                          Institutional development & Assessment of hydromet monitoring network, earl... &         30, 31 &       125000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & STRENGTHENING NATIONAL CAPABILITIES IN SOUTH SUDAN &                                                NaN &                          Institutional development & Strengthen hydrological monitoring for target a... &             31 &       150000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & STRENGTHENING NATIONAL CAPABILITIES IN SOUTH SUDAN &                                                NaN &                          Institutional development & Improving the capacity of South Sudan to genera... &             31 &       320000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & STRENGTHENING NATIONAL CAPABILITIES IN SOUTH SUDAN &                                                NaN &                          Institutional development & Develop pilot actions for community-level, impa... &             31 &       100000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & STRENGTHENING NATIONAL CAPABILITIES IN SOUTH SUDAN &                                                NaN &                          Institutional development & Upgrade of tele-conferencing facilities (South ... &             31 &        20000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & STRENGTHENING NATIONAL CAPABILITIES IN SOUTH SUDAN &                                                NaN &                          Institutional development & Strengthening National Risk Data Ecosystems in ... &             32 &       130000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &                  CREWS/RProj/12/East Africa & IMPROVED INTEGRATION OF GENDER AND VULNERABLE G... &                                                NaN & Gender-sensitive and vulnerable people inclusiv... & Integration of gender sensitivity and inclusion... &             32 &       150000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/RProj/15/Caribbean &  MHEWS Governance strengthened on a regional level & This component serves as an 'integrator,' where... & National mechanisms for more frequent multi-sec... &                                                NaN &             16 &      1804845 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/RProj/15/Caribbean & Disaster Risk Knowledge improved on a Regional,... &                                                NaN & National risk data ecosystems strengthened to i... &                                                NaN &             17 &       620000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/RProj/15/Caribbean & NMHS Service Provision, observation, monitoring... &                                                NaN & Marine Forecasting and related services strengt... &                                                NaN &             17 &      1614845 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/RProj/15/Caribbean & Warning dissemination and communication, prepar... &                                                NaN & Community-Based EWS strengthened. Warnings diss... &                                                NaN &             17 &       162500 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &                    CREWS/RProj/15/Caribbean & Warning dissemination and communication, prepar... &                                                NaN & Community-Based EWS strengthened. Warnings diss... &                                                NaN &             17 &       162500 &     Pillar 4 \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Institutional and human capacities in regional ... & Institutional and human capacities in regional ... &              7 &       100000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Institutional and human capacities in regional ... & Provide guidance to Kenya and Tanzania NMHSs, w... &              7 &        50000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Institutional and human capacities in regional ... & Provide guidance to the IOC in relation with th... &              8 &        50000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Institutional and human capacities in regional ... & Strengthen the existing Severe Weather Forecast... &              8 &       200000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Institutional and human capacities in regional ... & Enhance the regional cooperation as part of the... &              8 &       200000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Institutional and human capacities in regional ... & Provide guidance to national hydrological servi... &              8 &       150000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Institutional and human capacities in regional ... & Training on the use of custom indicators on Tar... &              8 &       500000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & NMHSs? service delivery improved, including the... & Provision of advisory services to heads of NMHS... &              8 &      1150000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & NMHSs? service delivery improved, including the... & Strengthening of real time flood hazard models ... &              8 &       125000 &     Pillar 2 \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Risk Information to guide early warning systems... & Developing a risk and flood impact modeling pla... &              9 &        75000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Risk Information to guide early warning systems... & Developing risk information to guide EWS in Com... &              9 &       175000 &     Pillar 1 \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Information and Communication Technology, inclu... & Provision of detailed guidance for common alert... &              9 &        50000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Information and Communication Technology, inclu... & Dissemination systems in Mozambique. Reviewing ... &              9 &       125000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Information and Communication Technology, inclu... & Dissemination systems in Comoros, Madagascar, M... &              9 &       200000 &     Pillar 3 \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Preparedness and response plans with operationa... & Establishing updated MoUs between the main agen... &              9 &        75000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Preparedness and response plans with operationa... & Establishing updated MoUs between the main agen... &              9 &       125000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Reviewing best practices in disseminating early... & Diagnostic and recommendations on multi-hazard ... &              9 &       350000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Gender-sensitive training, capacity building pr... & Gender-sensitive programming Identification of ... &          9, 10 &       100000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Gender-sensitive training, capacity building pr... & Gender-sensitive implementation. Provide adviso... &             10 &       100000 & Cross-Pillar \\
Climate Risk and Early Warning Systems (CREWS) &       CREWS/RProj07/South West Indian Ocean &                                                NaN &                                                NaN & Gender-sensitive training, capacity building pr... & Gender-sensitive monitoring. Ensure monitoring ... &             10 &       100000 & Cross-Pillar \\
\end{longtable}

